DISTA-Net: Dynamic Closely-Spaced Infrared Small Target Unmixing

Resolving closely-spaced small targets in dense clusters presents a significant challenge in infrared imaging, as the overlapping signals hinder precise determination of their quantity, sub-pixel positions, and radiation intensities. While deep learning has advanced the field of infrared small target detection, its application to closely-spaced infrared small targets has not yet been explored. This gap exists primarily due to the complexity of separating superimposed characteristics and the lack of an open-source infrastructure. In this work, we propose the Dynamic Iterative Shrinkage Thresholding Network (DISTA-Net), which reconceptualizes traditional sparse reconstruction within a dynamic framework. DISTA-Net adaptively generates convolution weights and thresholding parameters to tailor the reconstruction process in real time. To the best of our knowledge, DISTA-Net is the first deep learning model designed specifically for the unmixing of closely-spaced infrared small targets, achieving superior sub-pixel detection accuracy. Moreover, we have established the first open-source ecosystem to foster further research in this field. This ecosystem comprises three key components: (1) CSIST-100K, a publicly available benchmark dataset; (2) CSO-mAP, a custom evaluation metric for sub-pixel detection; and (3) GrokCSO, an open-source toolkit featuring DISTA-Net and other models. Our code and dataset are available at https://github.com/GrokCV/GrokCSO.

==> iccv-final/0-authors.tex <==
% !TEX root = ../main.tex

% author names and IEEE memberships
\author{
  Shengdong~Han,
  Shangdong~Yang,
  Xin~Zhang,
  Yuxuan~Li,
  Xiang~Li,
  % Renke~Kou,
  % Tianlin~Zhang,
  % Huan~Wang,
  % Kang~Ni,
  % Miao~Li,
  % Kehua~Guo,
  Jian~Yang,
  Ming-Ming~Cheng,
  Yimian~Dai

  \thanks{
    This work was supported by
      % 青基
      the National Natural Science Foundation of China
      (62301261, % 我
      % 杨尚东老师
      62206133,
      % 翔哥
      % 62206134,
      % 郭克华老师
      62472443,
      % 杨健老师
      U24A20330, 62361166670),
    % 博后面上
    % the China Postdoctoral Science Foundation (2021M701727),
    % 杨尚东老师
    Research Fund of Guangxi Key Lab of Multi-source Information Mining \& Security (MIMS22-01).
    %\emph{The first two authors contributed equally to this work. (Corresponding author: Shangdong Yang and Yimian Dai)}
    \emph{(Corresponding author: Yimian Dai)}
    }

  % 南邮
\thanks{
  Shangdong Yang and Shengdong Han
  % and Kang Ni 
  are with the School of Computer Science, Nanjing University of Posts and Telecommunications, Nanjing, China. Shangdong Yang is also with the Guangxi Key Lab of Multi-Source Information Mining and Security, Guangxi Normal University, Guilin, China.
    (e-mail:
    \href{mailto:sdyang@njupt.edu.cn}{sdyang@njupt.edu.cn});
    \href{mailto:hsdshengdong.han@gmail.com}{hsdshengdong.han@gmail.com}).
    % \href{mailto:ycy\_0818@163.com}{ycy\_0818@163.com};
    % \href{mailto:sdyang@njupt.edu.cn}{tznikang@njupt.edu.cn}
  }

  %
  % \thanks{
  %   Renke Kou is with School of Computer Science and Engineering, Central South University, Changsha 410083, China.
  %   (e-mail: \href{mailto:guokehua@csu.edu.cn}{guokehua@csu.edu.cn}).
  % }

 % 科大
 %  \thanks{
 %    Miao Li is with National University of Defense Technology (NUDT), Changsha, 410003, China.
 %    (e-mail: \href{mailto:lm8866@nudt.edu.cn}{lm8866@nudt.edu.cn}).
 %  }
  
 % % 科大
 %  \thanks{
 %    Xin Zhang is with National University of Defense Technology (NUDT), Changsha, 410003, China.
 %    (e-mail: \href{mailto:zhangxin21@nudt.edu.cn}{zhangxin21@nudt.edu.cn}).
 %  }

  %
  \thanks{
    Tianlin Zhang is with Luoyang Institute of Electro-optical Equipment, AVIC, Luoyang, 471000.
    (e-mail: \href{mailto:zhangtianlin17@mails.ucas.ac.cn}{zhangtianlin17@mails.ucas.ac.cn}).
  }

  % 中南
  \thanks{
    Kehua Guo is with School of Computer Science and Engineering, Central South University, Changsha 410083, China.
    (e-mail: \href{mailto:guokehua@csu.edu.cn}{guokehua@csu.edu.cn}).
  }

  % 南理工
  % \thanks{
  %   Jian Yang and Yimian Dai are with PCA Lab, Key Lab of Intelligent Perception and Systems for High-Dimensional Information of Ministry of Education, and Jiangsu Key Lab of Image and Video Understanding for Social Security, School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China.
  %   (e-mail:
  %   %\href{mailto:qun.dai.grokcv@gmail.com}{qun.dai.grokcv@gmail.com};
  %   %\href{mailto:wanghuanphd@njust.edu.cn}{wanghuanphd@njust.edu.cn};
  %   \href{mailto:csjyang@njust.edu.cn}{csjyang@mail.njust.edu.cn};
  %   \href{mailto:yimian.dai@gmail.com}{yimian.dai@gmail.com}.
  % }

  % % 南开
  % \thanks{
  % Xiang Li is with IMPlus@PCALab \& TMCC, CS, Nankai University. He also holds a position at the NKIARI, Shenzhen Futian. (e-mail:
  % \href{mailto:xiang.li.implus@nankai.edu.cn}{xiang.li.implus@nankai.edu.cn}).
  % }

  % 南开
  \thanks{
  Jian Yang and Yimian Dai are with VCIP, College of Computer Science, Nankai University. (e-mail:
  \href{mailto:csjyang@nankai.edu.cn}{csjyang@nankai.edu.cn};
  \href{mailto:yimian.dai@gmail.com}{yimian.dai@gmail.com})
  }
  
  % % 西交大
  % \thanks{Yan Yang is with the School of Mathematics and Statistics, Xi'an Jiaotong University, Xi'an, Shaanxi, 710049, P. R. China
  %   (e-mail: \href{mailto:yangyan@xjtu.edu.cn}{yangyan@xjtu.edu.cn}).
  % }
}

==> iccv-final/9-biography.tex <==
% !TEX root = ../main.tex

% Shengdong Han
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Shengdong_Han}}]{Shengdong Han} received the B.S. degree in software engineering from Wuhan University of Science and Technology in 2022. He is currently pursuing his master's degree in Electronic Information at Nanjing University of Posts and Telecommunications. His research interests include machine learning and computer vision.
\end{IEEEbiography}

% Shangdong Yang
\begin{IEEEbiography}[{
  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Shangdong_Yang}}]{Shangdong Yang} Shangdong Yang received the B.S. degree in automation from Southwest Jiaotong University, Chengdu, China, in 2013, and the Ph.D. degree in computer science and technology from Nanjing University, Nanjing, China, in 2020. He is currently an Assistant Professor with the School of Computer Science, Nanjing University of Posts and Telecommunications, Nanjing, and also a Project Moderator with Guangxi Key Lab of MultiSource Information Mining and Security, Guangxi Normal University, Guilin, China. His research interests include reinforcement learning and machine learning.
\end{IEEEbiography}



% Xin Zhang
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Xin_Zhang}}]{Xin Zhang} is currently pursuing his Ph.D. degree in information and communication engineering with the National University of Defense Technology (NUDT), Changsha, China. His research interests include infrared small target detection and deep learning.
\end{IEEEbiography}

% Miao Li
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Miao_Li}}]{Miao Li} received the M.E. and Ph.D. degrees from the National University of Defense Technology (NUDT) in 2012 and 2017, respectively. He is currently an Associate Professor with the College of Electronic Science and Technology, NUDT. His current research interests include infrared dim and small target detection.
\end{IEEEbiography}

% % Chunyang Yuan
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/ChunyangYuan}}]{Chunyang Yuan} received the B.S degree in energy and power engineering from Henan Polytechnic University, Henan, China, in 2021. He is currently pursuing a master's degree in Computer Science and Technology at Nanjing University of Posts and Telecommunications, Nanjing, China. His research interests include machine learning, SAR image processing, and computer vision.
% \end{IEEEbiography}

% 杨燕
% \begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Yan_Yang_Crop}}]{Yan Yang} received the Bachelor degree in school of mathematics and information science from the Shaanxi Normal University, China, in 2014. She received her PhD degree in the school of mathematics and statistics of Xi'an Jiaotong University in 2022. She is currently an assistant professor with School of Mathematics and Statistics,  Xian Jiaotong University.
%   Her research interests include image processing, medical imaging, and machine learning.
%   \end{IEEEbiography}

% Yuxuan Li
% \begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Yuxuan-Crop}}]{Yuxuan Li} is currently a Ph.D. student at the Department of Computer Science, Nankai University, China.
%   He graduated from University College London (UCL) with a first-class degree in Computer Science. He was the champion of the Second Jittor Artificial Intelligence Challenge in 2022, was awarded 2nd place in Facebook Hack-a-Project in 2019 and was awarded 2nd place in the Greater Bay Area International Algorithm Competition in 2022. His research interests include neural architecture design, and remote sensing object detection. 
% \end{IEEEbiography}





% % Xiang Li
% \begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/biography/Xiang_Li}}]{Xiang Li} is an Associate Professor in College of Computer Science, Nankai University. He received the PhD degree from the Department of Computer Science and Technology, Nanjing University of Science and Technology (NJUST) in 2020. There, he started the postdoctoral career in NJUST as a candidate for the 2020 Postdoctoral Innovative Talent Program. In 2016, he spent 8 months as a research intern in Microsoft Research Asia, supervised by Prof. Tao Qin and Prof. Tie-Yan Liu. He was a visiting scholar at Momenta, mainly focusing on monocular perception algorithm. His recent works are mainly on: neural architecture design, CNN/Transformer, object detection/recognition, unsupervised learning, and knowledge distillation. He has published 20+ papers in top journals and conferences such as TPAMI, CVPR, NeurIPS, etc.
% \end{IEEEbiography}

% % Huan Wang
% \begin{IEEEbiography}[{
% \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Huan_Wang}}]{Huan Wang} received B.S. degree in computer science from the Jiangsu university of Science and Technology, Zhen Jiang, China. He received the Doctor degree in pattern recognition and intelligent systems from Nanjing University of Science and Technology (NJUST), Nanjing, China. He is currently an associate professor with the School of Computer Science and Engineering, NJUST. He has authored over 40 scientifific papers in image processing, computer vision, pattern recognition, and artifificial intelligence. His current research interests include pattern recognition, robot vision and image processing.
% \end{IEEEbiography}

% Tianlin Zhang
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Tianlin-Zhang}}]{Tianlin Zhang} received the B.S. degree from the Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2017, and the Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, China, in 2023. He is currently an Engineer with Luoyang Institute of Electro-optical Equipment. His research interests include remote sensing image processing.

\end{IEEEbiography}

% Kehua Guo
\begin{IEEEbiography}[{
\includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Kehua-Guo}}]{Kehua Guo} Kehua Guo (M'13) received the Ph.D. degree in Computer Science and Technology from Nanjing University of Science and Technology, Nanjing, China, in 2008. He is currently a professor with Central South University, Changsha, China. He has served as a Guest Editor, Workshop Chair, Publicity Chair, Technical Program Committee Member, and Reviewer of international journals/conference proceedings. His research interests include artificial intelligence, big data, and image processing.
\end{IEEEbiography}

% Jian Yang
\begin{IEEEbiography}[{  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/biography/Jian_Yang}}]{Jian Yang} received the PhD degree from Nanjing University of Science and Technology (NJUST) in 2002, majoring in pattern recognition and intelligence systems. From 2003 to 2007, he was a Postdoctoral Fellow at the University of Zaragoza, Hong Kong Polytechnic University and New Jersey Institute of Technology, respectively. From 2007 to present, he is a professor in the School of Computer Science and Technology of NJUST. Currently, he is also a visiting distinguished professor in the College of Computer Science of Nankai University. His papers have been cited over 50000 times in the Google Scholar. His research interests include pattern recognition and computer vision. Currently, he is/was an associate editor of Pattern Recognition, Pattern Recognition Letters, IEEE Trans. Neural Networks and Learning Systems, and Neurocomputing. He is a Fellow of IAPR.
\end{IEEEbiography}

% Yimian Dai
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/biography/Yimian_Dai}}]{Yimian Dai} 
(Member, IEEE) received the B.E. degree in information engineering and the Ph.D. degree in signal and information processing from Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2013 and 2020, respectively.
From 2021 to 2024, he was a Postdoctoral Researcher with the School of Computer Science and Engineering, Nanjing University of Science and Technology, Nanjing, China. 
He is currently an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China.
His research interests include computer vision, deep learning, and their applications in remote sensing.
For more information, please visit the link (\href{https://yimian.grokcv.ai/}{https://yimian.grokcv.ai/}).

% During his Ph.D. study, he was a visiting scholar at the Department of Computer Science, University of Copenhagen, Denmark, under the supervision of Prof. Fabian Gieseke from March 2018 to September 2018, and at the Department of Computer Science, University of Arizona, USA, under the supervision of Prof. Kobus Barnard from October 2018 to October 2020.
% Since 2025, he has been an Associate Professor with the College of Computer Science, Nankai University, Tianjin, China. His research interests include computer vision, deep learning, and their applications in remote sensing, with a particular focus on developing advanced object detection algorithms to address real-world challenges.
% received the Ph.D. degree in signal and information processing from Nanjing University of Aeronautics and Astronautics, Nanjing, China, in 2021, during which he honed his research skills as a visiting Ph.D. student at the University of Copenhagen and the University of Arizona between March 2018 and October 2020. Since 2021, he has been with the School of Computer Science and Engineering, Nanjing University of Science and Technology (NJUST), Nanjing, where he is currently an Assistant Researcher. His research interests include remote sensing, computer vision, and deep learning, with a focus on developing algorithms for object detection, data assimilation, and computational imaging to tackle real-world challenges. He has authored more than 20 peer-reviewed journal and conference papers such as IJCV, TGRS, TAES, etc.
\end{IEEEbiography}
